Scaling Optimization Over Uncertainty via Compilation

Probabilistic inference is fundamentally hard, yet many tasks require optimization on top of inference, which is even harder. We present a new optimization-via-compilation strategy to scalably solve a certain class of such problems. In particular, we introduce a new intermediate representation (IR), binary decision diagrams weighted by a novel notion of branch-and-bound semiring, that enables a scalable branch-and-bound based optimization procedure. This IR automatically factorizes problems through program structure and prunes suboptimal values via a straightforward branch-and-bound style algorithm to find optima. Additionally, the IR is naturally amenable to staged compilation, allowing the programmer to query for optima mid-compilation to inform further executions of the program. We showcase the effectiveness and flexibility of the IR by implementing two performant languages that both compile to it: dappl and pineappl. dappl is a functional language that solves maximum expected utility problems with first-class support for rewards, decision making, and conditioning. pineappl is an imperative language that performs exact probabilistic inference with support for nested marginal maximum a posteriori (MMAP) optimization via staging.

==> appendices/optimization-via-compilation/additional-problems.tex <==
\subsection{An additional problem for BBIR representation}\label{subsec:sensitivity}

The \textit{sensitivity} of a probabilistic program  
measures the degree to which the inputs to a program may affect the output.
A main application is in algorithmic stability, in 
which we want to diagnose which configurations of an algorithm are most stable 
under varying input~\citep{aguirre2021pre}.
This sensitivity is often computed by bounding a notion of distance between two
possible distributions, such as the total variation distance:

\begin{definition}[Total variation distance~\citep{levin2017markov}]
  The total variation (TV) distance between two distributions 
  $\mu_1, \mu_2$ over the same finite set of random variables $X$
  is $TV(\mu_1, \mu_2) \triangleq \sum_{x \in X} \frac{|\mu_1(x)-\mu_2(x)|}{2}$. 
\end{definition}

In the case of a Boolean formula $\varphi$
% and a weight function
% $w : lits(\varphi) \to [0,1]$, it is known
% that $\AMC(\varphi, w)$ 
the AMC can
specify a distribution on the models of $\varphi$ with an appropriate weight 
function~\citep{de2007problog,holtzen2020scaling}. With this in mind, 
we can consider a discrete probabilistic program 
with a set
$I$ of Boolean inputs. The output of this program will be a 
distribution over models of the program satisfying the input. 

\citet{aguirre2021pre} consider the problem of bounding the expected
sensitivity of a probabilistic program.  In this setting it is 
also interesting to ask: what is the \textit{maximum}
sensitivity of a probabilistic program? This problem can be captured 
by the following BBIR where $(\{\varphi\}, I, w)$

\begin{enumerate}[leftmargin=*]
  \item $\varphi$ is the compiled probabilistic program as a Boolean formula,
  following existing strategies in the literature~\citep{holtzen2020scaling,de2007problog,saad2021sppl},
  \item $I$ the input variables,
  \item $w$ the weight function with codomain in the real branch-and-bound semiring
  $\R$ as per the previous example.
\end{enumerate}

Then the maximum probabilistic sensitivity problem will be:
\begin{equation}
  \begin{split}
  \mathrm{Sens}{(\{\varphi\}, I, w)} 
  &= \max_{(i,j) \in inst(I) \times inst(I)} TV(\varphi|_i, \varphi|_j).
  % & = \max_{(i,j) \in inst(I) \times inst(I)} \sum_{m \models \varphi|_i \lor \varphi|_j}
  %   \frac{|\Pr[\{m \models \varphi|_i\}] -\Pr[\{m \models \varphi|_j\}]|}{2}
\end{split}
\end{equation}

==> figs/pineappl-expr-relation.tex <==
\begin{figure}
\begin{mdframed}
  {\footnotesize
  \begin{align*}
    \infer[var/\top]
    {
        x[\sigma] = \top
    }
    {
        \sigma(x) = \top
    }
    \infer[var/\bot]
    {
        x[\sigma] = \bot
    }
    {
        \sigma(x) = \bot
    }
    \infer[\neg/\top]
    {
        \neg e[\sigma] = \bot
    }
    {
        e[\sigma] = \top
    }
    \infer[\neg/\bot]
    {
        \neg e[\sigma] = \top
    }
    {
        e[\sigma] = \bot
    }
  \end{align*}
  \begin{align*}
    \infer[\land/\top\top]
    {
        (e_1 \land e_2)[\sigma] = \top
    }
    {
        e_1[\sigma] = \top
        & e_2[\sigma] = \top
    }
    \infer[\land/\top\bot]
    {
        (e_1 \land e_2)[\sigma] = \bot
    }
    {
        e_1[\sigma] = \top
        & e_2[\sigma] = \bot
    }
  \end{align*}
  \begin{align*}
    \infer[\land/\bot\top]
    {
        (e_1 \land e_2)[\sigma] = \bot
    }
    {
        e_1[\sigma] = \bot
        & e_2[\sigma] = \top
    }
    \infer[\land/\bot\bot]
    {
        (e_1 \land e_2)[\sigma] = \bot
    }
    {
        e_1[\sigma] = \bot
        & e_2[\sigma] = \bot
    }
  \end{align*}
  \begin{align*}
    \infer[\lor/\top\top]
    {
        (e_1 \lor e_2)[\sigma] = \top
    }
    {
        e_1[\sigma] = \top
        & e_2[\sigma] = \top
    }
    \infer[\lor/\top\bot]
    {
        (e_1 \lor e_2)[\sigma] = \top
    }
    {
        e_1[\sigma] = \top
        & e_2[\sigma] = \bot
    }
  \end{align*}
  \begin{align*}
    \infer[\lor/\bot\top]
    {
        (e_1 \lor e_2)[\sigma] = \top
    }
    {
        e_1[\sigma] = \bot
        & e_2[\sigma] = \top
    }
    \infer[\lor/\bot\bot]
    {
        (e_1 \lor e_2)[\sigma] = \bot
    }
    {
        e_1[\sigma] = \bot
        & e_2[\sigma] = \bot
    }
  \end{align*}
  }
\end{mdframed}
\caption{Expression evaluation relation}
\label{fig:pineappl-expr-eval}
\end{figure}

==> sections/pineappl_bbir.tex <==
\begin{figure}
  \centering
  \scalebox{0.9}{
  \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]
      \def\lvl{20pt}

    \node (root) at (0, 0) [bddnode] {$\bigoplus$};
    \node at ($(root) + (0bp, 15bp)$) {{\color{gray} 0.75}};

    \node (mul1) at ($(root) + (-100bp, -\lvl)$) [bddnode] {$\bigotimes$};
    \node at ($(mul1) + (-23bp, 0)$) {{\color{gray} 0.675}};
    \node (mul2) at ($(root) + (100bp, -\lvl)$) [bddnode] {$\bigotimes$};
    \node at ($(mul2) + (23bp, 0)$) {{\color{gray} 0.075}};

    \node[bddformula] (term5) at ($(mul1) + (50bp, -\lvl)$) {$0.9$};
    \node[bddformula] (term6) at ($(mul2) + (-50bp, -\lvl)$) {$0.1$};

    \node (cup) at ($(mul1) + (-10bp, -\lvl)$) [bddnode] {$\sqcup$};
    \node at ($(cup) + (-20bp, 0)$) {{\color{gray} 0.75}};
    \node (cup2) at ($(mul2) + (10bp, -\lvl)$) [bddnode] {$\sqcup$};
    \node at ($(cup2) + (20bp, 0)$) {{\color{gray} 0.75}};


    \node[bddformula] (term1) at ($(cup) + (-50bp, -\lvl)$) {$\Pr[\texttt{boots}] = 0.75$};
    \node[bddformula] (term2) at ($(cup) + (50bp, -\lvl)$) {$\Pr[\overline{\texttt{boots}}] = 0.25$};

    \node[bddformula] (term3) at ($(cup2) + (-50bp, -\lvl)$) {$\Pr[\texttt{boots}] = 0.75$};
    \node[bddformula] (term4) at ($(cup2) + (50bp, -\lvl)$) {$\Pr[\overline{\texttt{boots}}] = 0.25$};

    \begin{scope}[on background layer]
      \draw [highedge] (root) -- (mul1) ;
      \draw [highedge] (root) -- (mul2);
      \draw [highedge] (mul1) -- (term5);
      \draw [highedge] (mul2) -- (term6);
      \draw [highedge] (mul1) -- (cup);
      \draw [highedge] (mul2) -- (cup2);
      \draw [highedge] (cup) -- (term1);
      \draw [highedge] (cup) -- (term2);
      \draw [highedge] (cup2) -- (term3);
      \draw [highedge] (cup2) -- (term4);
    \end{scope}
    \end{tikzpicture}
  }
\caption{Branch-and-bound circuit of the MMAP query over Equation~\ref{eq:partial-pineappl}.}
\label{fig:bbir-pineappl}
\end{figure}
